Table Enrichment System for Machine Learning

Data scientists are constantly facing the problem of how to improve prediction accuracy with insufficient tabular data. We propose a table enrichment system that enriches a query table by adding external attributes (columns) from data lakes and improves the accuracy of machine learning predictive models. Our system has four stages, join row search, task-related table selection, row and column alignment, and feature selection and evaluation, to efficiently create an enriched table for a given query table and a specified machine learning task. We demonstrate our system with a web UI to show the use cases of table enrichment.

==> augmentation.tex <==
\subsection{Row and column alignment}
\label{sec:row:column:alignment}


%\subsection{Join row mapping}
%After the task-related table selection,
%the number of candidate join tables will be filtered to thousands of rows with hundreds of tables.
The next step is to map these rows and join them to the query table.
We join the candidate rows and align the rows if they are from the same table.
Note that for each query row, it may retrieve multiple join rows from the same target table.
In this case, we map the row with the highest similarity score since a target table usually only has one matching row (entity) to a query row.

\begin{comment}
The example in figure \ref{fig:overall-example} shows an example of joining the candidate rows to the query table.
An enriched table is created once the join row mapping is finished.
We can train the predictive model with this enriched table, and
this is a baseline method in our experiment.
\end{comment}


%\subsection{Column aggregation}
As shown in Table \ref{fig:overall-example}, the enriched part of the table will be sparse in most cases,
which means the enriched table may contain a large number of columns with many empty values.
This is because different query rows may not join the same target table, 
and the row number of a target table may also differ from the query table.
The size of enriched columns determines the processing time,
and the empty values will decrease the performance of the feature selection algorithm and predictive models.


To achieve high performance with a short processing time,
we propose to aggregate columns to decrease the column numbers and impute most of the empty values.
\begin{comment}
This task is related to schema matching, table union, and table stitching \cite{schema-matching, valentine-schema-matching, table-union-search, table-stitch}.
There are two categories of methods to match two or more tables.
One is \textit{Column name-based method} that matches two according to the syntactic or semantic overlaps between their column names.
The other is \textit{Column value-based method} to match two or more tables with their data types, values, and value distributions.

We use a column name-based method that defines two target tables that can be aggregated when the column names have an overlap above a given threshold,
for the following two reasons:
(a) \textbf{Correctness}. Taking overlap with the same column name is a strong method that can ensure the correctness of column aggregation. 
It will be a positive affection on the accuracy of the ML task if we aggregate the irrelated columns.
(b) \textbf{Efficacy}. Another reason is that the candidate number of tables is at least thousands in our problem,
we need a lightweight method that can allow us to process pair-wise matching efficiently.
Most of the complicated value-based methods are not available for large-scale data.
\end{comment}
We use a column name-based method that aggregates two columns when their column names have an overlap above a given threshold.
Specifically,
for each candidate table, we take the Jaccard similarity in Equation \ref{equ:jac} to the rest of the candidate tables
and aggregate them if their similarity is above a pre-defined threshold. 
Having more compact enriched columns does not always result in better accuracy on the final ML task, so
%It will also create noise if we set a small $\tau$ and aggregate too many tables together.
the threshold should be tuned in practice.
During aggregation, the values may be conflicted at the same position of rows, 
and we aggregate the conflicted values by string concatenation or averaging numerical values. 
For numeric values, we also detect and align the different units such as ``65.4\$'' and ``1K€'' with rule-based transformations.

Figure \ref{fig:overall-example} also shows the enrichment result after column aggregation. We can see that it is much cleaner with less empty values than
the result of join row mapping.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{tata/images/demo1-crop.pdf}
  \includegraphics[width=\linewidth]{tata/images/demo2-crop.pdf}
   \includegraphics[width=\linewidth]{tata/images/demo3-crop.pdf}
   \caption{Web UI of the table enrichment demo. The steps of our guide demonstration are marked in red circle.}
  \label{fig:demo}
\end{figure}



\subsection{Feature selection}
Finally, we process feature selection to filter noisy columns.
%There are three types of feature selection methods: filter, wrapper, and embedded \cite{fs-survey}.
The feature selection algorithms were built with 
the sklearn \footnote{https://scikit-learn.org/stable/modules/feature\_selection.html} 
with the default setting, which included: 
F-value, Forward selection, Backward selection, Recursive
Feature Elimination (RFE), Random forest, and Linear model with L1 regularization.
Our system offers several feature selection methods with 
and lets users tune and select the best one.


==> augmentation_alg.tex <==
\begin{algorithm}[t]
  \Input{candidate tables $T_{cand}$, local table $X_l$}
  \Output{augmented table}
  
  \State{$X_j \gets$ multi-join($X_l, T_{cand}$)}
  \State{$X_C \gets$ Clustering the extended columns in $X_j$}
  \State{$F \gets \emptyset$}
  \ForEach{cluster $x_c \in X_C$}{
    \State{Union and filter columns in $x_c$}
    \State{$F \gets$ union columns}
    }
  \State{Run feature selection algorithm on $F$ with $X_l$}
  \Return{augmented table with selected columns}
  \caption{Table Augmentation}
  \label{alg:augmentation}
\end{algorithm}

==> experiment.tex <==
\subsection{Experiment}
\label{sec:exp}

%\mysubsection{Setting}

\begin{comment}
\begin{table*}[t]
  \centering
  \caption{Datasets statistics}  
  \begin{tabular}{ |l|l|l|l| } 
    \hline
    Dataset & ML Task & Size \\
    \hline
    COMPANY & Company 13-category classification      & 73,935\\
    WALMART & Walmart product 31-category classification & 30,000\\
    AMAZON  & AMAZON toy product 39-category classification & 10,000 \\
    GAME   & Video game global sale regression          & 11,493\\
    MOVIE    & Movie IMDB score regression                      & 5,000\\
    CAR     & Car price regression                       & 200\\
    \hline
  \end{tabular}
  \label{tab:datasets}
\end{table*}

\mysubsection{Datasets}
\end{comment}

\begin{table}[t]
  \begin{center}
    \caption{ML scores and processing time GAME and AMAZON datasets.} 
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{|l|ccl|}\hline
                        \multicolumn{4}{|c|}{GAME} \\\hline
      Method           & MSE               & Improvement    & Time(s)  \\\hline
      No-enrich       & 0.603 $\pm$ 0.054 & -              &  -        \\ 
      %Join-corr-PCC (\cite{join-corr}) & 0.477 $\pm$ 0.052 & +20.89\%    &  664    \\
      %Join-corr-SCC (\cite{cocoa})   & 0.473 $\pm$ 0.076  &  +21.55\%   &  589\\
      Join        & 0.476 $\pm$ 0.067 & +21.06\%        &2546\\
      Join-align        & 0.471 $\pm$ 0.055 & +21.89\%        &1102\\
      Join-select       & 0.475 $\pm$ 0.043 & +21.22\%        &452\\
      Join-select-align & \textbf{0.466 $\pm$ 0.051} & \textbf{+22.72\%}        & \textbf{42}\\ \hline \hline 
                         \multicolumn{4}{|c|}{AMAZON} \\\hline
      Method (Baseline)       & F1                & Improvement   & Time(s)  \\\hline
      No-enrich       & 0.608 $\pm$ 0.053 & -         &-\\ 
      %Join-corr-PCC (\cite{join-corr})  &  0.599 $\pm$ 0.035  & -1.48\% & 787   \\
      %Join-corr-SCC (\cite{cocoa})   &   0.594 $\pm$ 0.044  &  -2.30\% & 899\\
      Join          & 0.582 $\pm$ 0.049 & -4.28\%   &2546\\
      Join-align        & 0.589 $\pm$ 0.036 & -3.12\%   &1102\\
      Join-select       & 0.617 $\pm$ 0.044 & +1.48\%   &103\\
      Join-select-align & \textbf{0.635 $\pm$ +0.047} &  \textbf{+4.44\%}   &\textbf{42}\\ \hline
    \end{tabular}
    }
    \label{tab:exp}
  \end{center}
\end{table}

We conducted an experiment to test both ML prediction accuracy and running time.
We used two query tables from Kaggle \cite{URL:kaggle}, GAME \footnote{{https://www.kaggle.com/gregorut/videogamesales}} 
with the task of sale prediction, and 
AMAZON \footnote{{https://www.kaggle.com/PromptCloudHQ/toy-products-on-amazon}} 
with the task of product classification.
For the target tables, we extracted 10M English-Language relational web tables from the WDC Web Table Corpora \cite{URL:WDC}.
Table \ref{tab:exp} reports the results.
For the ablation study, we also compared
\textit{Join} (Only join row search), 
\textit{Join-align} (join row search + row and column alignment) 
and \textit{Join-select} (join row search + task-related table selection).
We can see the full version of the proposed system \textit{Join-align-align} 
have the best performance improvement on ML prediction and have the shortest running time.



%We indexed all rows with string cells with the cell index, and also indexed the metadata attributes described in Section \label{sec:prob:state} into the table index.
\begin{comment}
COMPANY, \footnote{{https://www.kaggle.com/charanpuvvala/company-classification}},
WALMART, \footnote{{https://www.kaggle.com/promptcloud/walmart-product-data-2019}},


MOVIE, \footnote{{https://www.kaggle.com/carolzhangdc/imdb-5000-movie-dataset}},
and CAR, \footnote{{https://www.kaggle.com/goyalshalini93/car-data}}
from Kaggle \cite{URL:kaggle} 
with different ML prediction tasks on both regression and classification.  
The task descriptions and data size are described in Table \ref{tab:datasets}.



\mysubsection{Methods}
We had the following methods with a baseline method and several different versions of the proposed table enrichment method for the ablation study.
\begin{itemize}
    \item \textbf{Query-table}: 
    A baseline method that only trains and predicts on the query table without table enrichment.
    \item \textbf{Join-corr-PCC}
    A baseline method of \cite{join-corr} that retrieves the joinable table and select tables with Pearson correlation coefficient for linear ML models
    \item \textbf{Join-corr-SCC}
    A baseline method of \cite{cocoa} that retrieves the joinable table and select tables with Spearman’s correlation coefficient for non-linear ML models
    
    \item \textbf{Join}:
    Table enrichment method by only joining all rows after join row searching.
    \item \textbf{Join-align}:
    Table enrichment method by joining all rows and then aligning rows and columns without task-related table selection.
    \item \textbf{Join-select}:
    Table enrichment method by joining the task-related rows without row and column alignment.
    \item \textbf{Join-select-align}:
    The full version of our proposed table enrichment method.
\end{itemize}
\end{comment}

\begin{comment}
\mysubsection{Setting}
For the join row search, we used the "name" column in each query table as the query column.
For each query row, we set $k =$ [20, 40, 60, 80, 100] and $k=60$ as default to retrieve top-$k$ target rows from data lakes.
For task-related table selection, we set $m =$ [200, 400, 600, 800, 1000] and $m=600$ as default to select top-$m$ candidate tables.
We used Text 2, X + Y (e.g. "Video game sales") as the query text.
We used fastText to encode the strings as default and we also compare the results with that of BERT.
For row and column alignment, we set the threshold of Jaccard similarity as $\tau = [0.2, 0.4, 0.6, 0.8, 1]$ and the default is $\tau = 0.6$ between the column names of the two tables.
For feature selection, model selection, and training, we used the random forest model (non-linear) and linear model with L1 regularization with the default parameters in scikit-learn \cite{sklean}.
This is because the random forest and L1 regularization can automatically process feature selection when training.
We selected and reported the best score between them.


\mysubsection{Evaluation metrics}
For the accuracy evaluation,
we evaluated MSE on GAME and MOVIE datasets with MSE (mean square error), 
and RMSE (root mean square error) for the CAR dataset (since the car price is large).
We computed the macro-F1 for multi-classification tasks on COMPANY, WALMART, and AMAZON.
For each dataset, we processed 4-fold cross-validation and reported the average score of each method.
On the other hand, we also measured the end-to-end processing time to evaluate the efficiency.




\subsection{Experimental results}



\textbf{Can table enrichment improve the ML accuracy?}

Tables \ref{tab:exp:reg} and \ref{tab:exp:cls} reports the ML accuracy for regression and classification tasks, respectively. 
Note that in the regression task of Tables \ref{tab:exp:reg}, the smaller value means the better accuracy,
but in classification task of Tables \ref{tab:exp:cls}, the larger value means the better accuracy.
The ``improvement'' columns report the performance gain compared with the \textit{Query-table} method.
In both classification and regression tasks,
our full version method \textit{Join-select-align} had the best accuracy in all cases.
Compared with the \textit{Query-table} which is only trained by the original query table,
our method can bring more powerful feature that improves the accuracy up to 22.72\%.
For the correlation-based retrieving methods, \textit{Join-corr-PCC} and \textit{Join-corr-SCC},
our method also had better accuracy since the correlation limits the features,
while our method can optimize the features by model selection.
We also observed that sometimes the enriched columns of correlation-based methods are actually noise 
but correlated to the target column by coincidence. 
On the other hand, this rarely happened in our proposed method since the task-related table selection using
metadata that can select tables with similar topics.

We can also see that the values of improvement are different in different ML tasks.
The GAME and CAR dataset had a large improvement over about 17\% to 22\% while
the AMAZON and MOVIE had about 2\% to 4\% improvement, and the COMPANY and WALMART had an improvement less than 2\%.
For COMPANY and WALMART, the query table itself already achieved a high f1 score ($>0.8$) for classification,
and improving the accuracy on them is more difficult than other datasets. 
It is important to note that even a 1\%-2\% accuracy gain is incredible since it can also increase a large market profit.
We also observed the enriched table of the WALMART dataset because the target tables contain the data in 2015 but the WALMART has the products data in 2019
We found that different product names are joined to the WALMART dataset but contain similar terms of brands and categories.
This is an interesting insight that it is not necessarily to join the same entity to the query table.
Joining different entities with similar attributes (terms) can also improve the accuracy of the ML tasks.

For the ablation study, we first compared \textit{Join}, \textit{Join-align} and \textit{Join-select}.
We found that the task-related table selection has more impact than column alignment on accuracy. 
In the COMPANY and WALMART datasets, the accuracy decreased than the \textit{Query-table}.
This is because the candidate tables contain noise data without processing a task-related table selection.
Then, according to the results of \textit{Join-align}, \textit{Join-select} and \textit{Join-align-select}.
We found that the task-related table selection and column alignment have an interaction impact for better ML accuracy.

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-acc.pdf}
    \caption{Accuracy}
    \label{exp:cluster:f1:k}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-time.pdf}
    \caption{Runtime}
    \label{exp:cluster:f1:time:k}
  \end{subfigure}
  \caption{Varying $k$ in join row search, COMPANY, WALMART, and AMAZON. }
  \label{exp:CWA:k}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-acc.pdf}
    \caption{Accuracy}
    \label{exp:cluster:f1:m}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-time.pdf}
    \caption{Runtime}
    \label{exp:cluster:f1:time:m}
  \end{subfigure}
  \caption{Varying $m$ in task-related table selection, COMPANY, WALMART, and AMAZON.}
  \label{exp:CWA:m}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-acc.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:tau}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-time.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:tau}
  \end{subfigure}
  \caption{Varying $\tau$ in column alignment, COMPANY, WALMART, and AMAZON. }
  \label{exp:CWA:tau}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-acc-gm.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:k}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-time-gm.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:k}
  \end{subfigure}
  \caption{Varying $k$ in join row search, GAME and MOVIE. }
  \label{exp:GM:k}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-acc-gm.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:m}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-time-gm.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:m}
  \end{subfigure}
  \caption{Varying $m$ in task-related table selection, GAME and MOVIE.}
  \label{exp:GM:m}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-acc-gm.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:tau}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-time-gm.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:tau}
  \end{subfigure}
  \caption{Varying $\tau$ in column alignment, GAME and MOVIE.}
  \label{exp:GM:tau}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-acc-car.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:k}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-k-time-car.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:k}
  \end{subfigure}
  \caption{Varying $k$ in join row search, CAR}
  \label{exp:CAR:k}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-acc-car.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:m}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-m-time-car.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:m}
  \end{subfigure}
  \caption{Varying $m$ in task-related table selection, CAR}
  \label{exp:CAR:m}
\end{figure}

\begin{figure}[t]
  \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-acc-car.pdf}
    \caption{Accuracy}
    \label{exp:cluster:mse:tau}
  \end{subfigure}\begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[width=\linewidth]{exp/vary-tau-time-car.pdf}
    \caption{Runtime}
    \label{exp:cluster:mse:time:tau}
  \end{subfigure}
  \caption{Varying $\tau$ in column alignment, CAR}
  \label{exp:CAR:tau}
\end{figure}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.6\linewidth]{exp/feature_importance.pdf}
  \caption{GAME dataset}

  \centering
  \includegraphics[width=0.6\linewidth]{exp/feature_importance_amazon.pdf}
  \caption{AMAZON dataset}
 
  \caption{ Top-20 feature importance by the random forest model with the corresponding column names. 
  The blue bars are the columns from the query table and the red bars are enriched columns from the data lakes (WDC web tables).}
\label{fig:feature:importance}
\end{figure*}



\textbf{Can table enrichment have a short processing time?}

Let see the columns of "Time(s)" in Tables \ref{tab:exp:reg} and \ref{tab:exp:cls} that reports the runtime of each method.
There is no doubt that the \textit{Join-select-align} is the most efficient method with 6x to 72x speedup compared 
\textit{Join}.
This is because that the full version of the proposed method 
has both task-related table selection and column aggregation, which can greatly reduce the number of candidate data while processing.
This is mainly owned by the power of task-related table selection that reduces a large of candidate tables.
The method \textit{Join-align} also reduced about half of the processing time than \textit{Join}.
Combined with the accuracy results, we can say that the task-related table selection is an important stage
that largely speeds up the processing and increases the accuracy.
\textit{Join-corr-PCC} and \textit{Join-corr-SCC} can also further select candidate tables by ranking the correlation values of their columns,
but it is still slower than our method since they do not contain the processing of column aggregation, which can also extremely reduce the candidate columns to process.
Even the COMPANY dataset which contains 70k rows were finished in 100 seconds,
we conclude that the table enrichment solution has the ability to have a short processing time for most practical data science tasks with ML.

%\fixme{abulation study + enriched result sample, show different }

\textbf{Does putting ``task" into query text in task-related table selection works better?}

We evaluated the final accuracy scores with different query text patterns in task-related table selection. 
We also added a baseline query text pattern, Text 0 (X) (e.g. "video game" without ``sale"), to test the performance of adding ``task" into query text.
The results are reported in Tables \ref{tab:exp:reg} and \ref{tab:exp:cls} with the accuracy values and rank values.
We can see that Text 2 and Text 3 always have better accuracy on the top-1 or top-2 rank.
We also observed the selected tables and we found that adding the task "Y" into the query text can retrieve more related tables.
For example, we retrieved a table about game sales records with Text 2 but that table was not selected by Text 0.
On the other hand, Text 1 always ranked at the last part.
This is because the column names are sometimes insufficient.
The video game sales table has column names with "Game Name, Year, Genre, Sales".
Although the target Y is included, the ``Year" and ``Genre" may affect the encoded vectors to deviate from the topic of the video game.

\textbf{Which pre-train language model works better? fastText or BERT?}

The difference between fastText and BERT is that fastText is a word embedding model which always encodes the same word into the same vector.
However, BERT considers the context of the text so that the same word can be encoded into different vectors in different sentences. 
For example, the vector of "video" in "youtube video" and "video game" is different.
On the other hand, fastText also has the merit that it embeds vectors with sub-word, which can solve the out-of-vocabulary problem.
According to the results in Tables \ref{tab:exp:reg} and \ref{tab:exp:cls}, the performance of fastText and BERT are similar.
FastText was better than BERT in GAME, CAR, and COMPANY datasets while BERT was strong in others.





%and we recommend using \tata with these wrapper methods in practice

\textbf{Effect on varying parameters of $k$, $m$, and $\tau$.} 

We tested the performance of \textit{join-select-align} method with different parameters.
%We plot the results from the three classification datasets of COMPANY, WALMART, and AMAZON since both F1 scores and runtime have a similar value range.
Figures \ref{exp:CWA:k}, \ref{exp:GM:k} and \ref{exp:CAR:k} shows the results of varying $k$ in the join row search stage, 
we can see that the accuracy scores increased with the large $k$ since we have more probability to retrieve the valuable table for the ML task. 
The noise table will also increase with large $k$ but we have the 
task-related table selection to filter those data.
On the other hand, the processing time also increased linearly since more candidate tables lead to more computation.

Figures \ref{exp:CWA:m}, \ref{exp:GM:m} and \ref{exp:CAR:m} shows the results on varying $m$ in task-related table selection. 
In most cases, the accuracy decreased and runtime increased decreased with the growth of $m$.
This is because the ratio of the noise table increases and affects the performance of the ML model,
and large candidate tables also lead to more computation in the next stages.

Figure \ref{exp:CWA:tau}, \ref{exp:GM:tau} and \ref{exp:CAR:tau} shows the results on varying $\tau$ in column alignment. 
Note that smaller $\tau$ allows more tables and columns to be aggregated and create a more compact enriched table.
We can see that the accuracy first increased and then decrease with the change of $\tau$.
Different datasets have different peak values, such as AMAZON had a peak value of $\tau = 0.4$ while COMPANY and WALMART had the peak when $\tau = 0.6$.
Nevertheless, we conclude that the $\tau$ should be tuned according to the dataset since there is no uniform similarity threshold
for any kind of candidate table.
The runtime grows linearly with the large $\tau$ since more columns cause more processing time in the evaluation.









\textbf{Why table enrichment can improve ML performance?}
To answer this question, we take an insight to observe the enriched columns, the features (words) after feature extraction,
and the ranking of feature importance.
For the page limitation, we report the result of the GAME dataset and AMAZON datasets which are representative for regression and classification ML tasks.
Other datasets had similar results.
Figure \ref{fig:feature:importance} 
shows the top-20 feature importance with the column name from the enriched table. 
The blue bars are the columns from the query table and the red bars are enriched columns.
There are 8 features from the data lakes ranking in top-20.
This clearly shows the power of table enrichment that can contribute to the ML model for improving accuracy.

There are two reasons why our table enrichment can improve the ML performance.
The first which is also the most important reason is that table enrichment can \textbf{bring new information}.
The numeric values on ``Total Sales" from the external web tables are correlated with global sales in the GAME dataset;
The information of ``brand", ``reviews" and ``Description" can enrich the feature of new words within one-hot or TF-IDF vectorization, 
these new dimensions of words can better classify the products in AMAZON.
The second reason is the \textbf{data augmentation of samples}.
We know that the model may easy to overfit when the model learns the details and noise in the query table.
Therefore, even with no new information from the external tables, the different styles of presentation on the existed attribute can also help.
This is the case of enriched columns ``Game" and ``Title" for the original column "Name" for GAME datasets,
and the enriched ``product" for ``product\_name" in the AMAZON dataset.
For example, the model may learn the word weight equally when we only have the text of "Super Mario Bros",
but after table enrichment, the enriched parts contain the different styles of presentation such as ``mario II" and ``super mario".
And the model will realize the important word is ``mario" since it appears three times.
This can help to improve the accuracy since the games which contain ``mario" in their title may have similar values of global sales,
thus having a more accurate prediction.
\end{comment}


==> experiment_table.tex <==
\begin{table}[t]
  \begin{center}
    \caption{ML scores and processing time for regression tasks on GAME, MOVIE, and CAR datasets.} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|ccl|}\hline
                         \multicolumn{4}{|c|}{GAME} \\\hline
      Method           & MSE               & Improvement    & Time(s)  \\\hline
      Query-table       & 0.603 $\pm$ 0.054 & -              &  -        \\ 
      Join-corr-PCC (\cite{join-corr}) & 0.477 $\pm$ 0.052 & +20.89\%    &  664    \\
      Join-corr-SCC (\cite{cocoa})   & 0.473 $\pm$ 0.076  &  +21.55\%   &  589\\
      Join        & 0.476 $\pm$ 0.067 & +21.06\%        &2546\\
      Join-align        & 0.471 $\pm$ 0.055 & +21.89\%        &1102\\
      Join-select       & 0.475 $\pm$ 0.043 & +21.22\%        &452\\
      Join-select-align & \textbf{0.466 $\pm$ 0.051} & \textbf{+22.72\%}        & \textbf{42}\\ \hline \hline 
                         \multicolumn{4}{|c|}{MOVIE} \\\hline
      Method            & MSE               & Improvement    & Time(s)  \\\hline
      Query-table       & 0.902 $\pm$ 0.013 & -              & -\\ 
      Join-corr-PCC (\cite{join-corr}) & 0.901 $\pm$ 0.022 & +0.11\%    &  212    \\
      Join-corr-SCC (\cite{cocoa})   & 0.892 $\pm$ 0.035  &  +1.11\%   &  198\\
      Join          & 0.889 $\pm$ 0.015 & +1.44\%        &1895\\
      Join-align        & 0.893 $\pm$ 0.021 & +0.99\%        &1235\\
      Join-select       & 0.885 $\pm$ 0.017 & +1.88\%        &117\\
      Join-select-align & \textbf{0.883 $\pm$ 0.022} & \textbf{+2.11}\%        &\textbf{33}\\ \hline \hline 
                         \multicolumn{4}{|c|}{CAR} \\ \hline
      Method           & RMSE              & Improvement    & Time(s)  \\\hline
      Query-table       & 5526 $\pm$ 1223 & -              &-\\ 
      Join-corr-PCC (\cite{join-corr}) & 5333 $\pm$ 1202 & +3.49\%    &  2.44   \\
      Join-corr-SCC (\cite{cocoa})   & 5223 $\pm$ 989  &  +5.48\%   &  3.10\\
      Join          & 5044 $\pm$ 1345 & +8.72\%        &6.17\\
      Join-align        & 5156 $\pm$ 1024 & +6.69\%        &3.72\\
      Join-select       & 4778 $\pm$ 1127 & +13.54\%        &1.91\\
      Join-select-align & \textbf{4541 $\pm$ 1233} & \textbf{+17.82}\%        &\textbf{1.03}\\ \hline
    \end{tabular}
    }
    \label{tab:exp:reg}
  \end{center}
\end{table}

\begin{table}[t]
  \begin{center}
    \caption{ML scores and processing time for classification on COMPANY, WALMART, and AMAZON datasets.} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|ccl|}\hline
                         \multicolumn{4}{|c|}{COMPANY} \\\hline
      Method           & F1                & Improvement   & Time(s)  \\\hline
      Query-table       & 0.913 $\pm$ 0.035 & -             &  -        \\ 
      Join-corr-PCC (\cite{join-corr})  &  0.917 $\pm$ 0.043  & +0.44\% & 787   \\
      Join-corr-SCC (\cite{cocoa})   &   0.919 $\pm$ 0.056  &  +0.65\% & 899\\
      Join              & 0.916 $\pm$ 0.049 & +0.32\%       &6434\\
      Join-align        & 0.921 $\pm$ 0.027 & +0.87\%       &2435\\
      Join-select       & 0.924 $\pm$ 0.065 & +1.20\%       &357\\
      Join-select-align & \textbf{0.931 $\pm$ 0.046} & \textbf{+1.97\%}      &\textbf{100}\\ \hline \hline
                         \multicolumn{4}{|c|}{WALMART} \\\hline
      Method        & F1                & Improvement   & Time(s)  \\\hline
      Query-table       & 0.811 $\pm$ 0.013 & -             & -\\ 
      Join-corr-PCC (\cite{join-corr})  &  0.809 $\pm$ 0.015  & -0.25\% & 787   \\
      Join-corr-SCC (\cite{cocoa})   &   0.801 $\pm$ 0.024  &  -1.23\% & 899\\
      Join          & 0.774 $\pm$ 0.020 & -4.56\%       &5059\\
      Join-align        & 0.812 $\pm$ 0.015 & +0.12\%       &1640\\
      Join-select       & 0.815 $\pm$ 0.021 & +0.49\%       &277\\
      Join-select-align &  \textbf{0.820 $\pm$ 0.014} &  \textbf{+1.10\%}       & \textbf{66}\\ \hline \hline
                         \multicolumn{4}{|c|}{AMAZON} \\\hline
      Method (Baseline)       & F1                & Improvement   & Time(s)  \\\hline
      Query-table       & 0.608 $\pm$ 0.053 & -         &-\\ 
      Join-corr-PCC (\cite{join-corr})  &  0.599 $\pm$ 0.035  & -1.48\% & 787   \\
      Join-corr-SCC (\cite{cocoa})   &   0.594 $\pm$ 0.044  &  -2.30\% & 899\\
      Join          & 0.582 $\pm$ 0.049 & -4.28\%   &2546\\
      Join-align        & 0.589 $\pm$ 0.036 & -3.12\%   &1102\\
      Join-select       & 0.617 $\pm$ 0.044 & +1.48\%   &103\\
      Join-select-align & \textbf{0.635 $\pm$ +0.047} &  \textbf{+4.44\%}   &\textbf{42}\\ \hline
    \end{tabular}
    }
    \label{tab:exp:cls}
  \end{center}
\end{table}


\begin{table*}[t]
  \begin{center}
    \caption{Compare Text patterns and encoders in task-related table selection for regression tasks of GAME, MOVIE, and CAR datasets} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
      Query text                    &Encoder  & \multicolumn{2}{|c|}{GAME (RMSE \& Rank)}   & \multicolumn{2}{|c|}{MOVIE (MSE \& Rank)}  & \multicolumn{2}{|c|}{CAR (MSE \& Rank)} \\\hline
      Text 0 (X)                    &fastText & 0.486$\pm$ 0.033  & 4   & 0.886$\pm$ 0.011 & 4&  4665$\pm$ 1543 &5\\
      Text 1 (column names)         &fastText & 0.511$\pm$ 0.064  & 6   & 0.891$\pm$ 0.017 & 5&  4688$\pm$ 1653 &6     \\ 
      Text 2 (X + y)                &fastText & 0.466$\pm$ 0.051  & 1   & 0.883$\pm$ 0.022 & 3&  4541$\pm$ 1233 &3  \\
      Text 3 (X + y + "prediction") &fastText & 0.471$\pm$ 0.055  & 2   & 0.876$\pm$ 0.021 & 2&  4336$\pm$ 1147 &1     \\ 
      Text 0  (X)                   &Bert     & 0.523$\pm$ 0.061  & 7   & 0.894$\pm$ 0.019 & 8&  4791$\pm$ 1442 &7     \\ 
      Text 1  (column names)        &Bert     & 0.531$\pm$ 0.059  & 8   & 0.893$\pm$ 0.026 & 7&  4912$\pm$ 1231 &8 \\
      Text 2  (X + y)               &Bert     & 0.486$\pm$ 0.054  & 5   & 0.892$\pm$ 0.033 & 6&  4556$\pm$ 1651 &4     \\ 
      Text 3 (X + y + "prediction") &Bert     & 0.485$\pm$ 0.066  & 3   & 0.874$\pm$ 0.014 & 1&  4419$\pm$ 1798 &2\\\hline
    \end{tabular}
    }
    \label{tab:exp:textpe:reg}
  \end{center}
\end{table*}

\begin{table*}[t]
  \begin{center}
    \caption{Compare Text patterns and encoders in task-related table selection for classification tasks of COMPANY, WALMART, and AMAZON datasets} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
      Query text                    &Encoder  & \multicolumn{2}{|c|}{COMPANY (F1 \& Rank)}   & \multicolumn{2}{|c|}{WALMART (F1 \& Rank)}  & \multicolumn{2}{|c|}{AMAZON (F1 \& Rank)} \\\hline
      Text 0 (X)                    &fastText & 0.916$\pm$ 0.055  & 5   & 0.803$\pm$ 0.015 & 6&  0.615$\pm$ 0.056 &8\\
      Text 1 (column names)         &fastText & 0.911$\pm$ 0.042  & 6   & 0.802$\pm$ 0.018 & 7&  0.615$\pm$ 0.061 &7     \\ 
      Text 2 (X + y)                &fastText & 0.922$\pm$ 0.048  & 1   & 0.816$\pm$ 0.014 & 2&  0.625$\pm$ 0.047 &3  \\
      Text 3 (X + y + "prediction") &fastText & 0.918$\pm$ 0.055  & 3   & 0.814$\pm$ 0.020 & 3&  0.631$\pm$ 0.043 &1     \\ 
      Text 0  (X)                   &Bert     & 0.910$\pm$ 0.064  & 7   & 0.808$\pm$ 0.011 & 5&  0.622$\pm$ 0.046 &4     \\ 
      Text 1  (column names)        &Bert     & 0.908$\pm$ 0.053  & 8   & 0.799$\pm$ 0.017 & 8&  0.629$\pm$ 0.055 &2 \\
      Text 2  (X + y)               &Bert     & 0.921$\pm$ 0.033  & 2   & 0.818$\pm$ 0.019 & 1&  0.618$\pm$ 0.061 &6     \\ 
      Text 3 (X + y + "prediction") &Bert     & 0.916$\pm$ 0.047  & 4   & 0.810$\pm$ 0.014 & 4&  0.621$\pm$ 0.039 &5\\\hline
    \end{tabular}
    }
    \label{tab:exp:textpe:cls}
  \end{center}
\end{table*}





\begin{comment}
\begin{table}[t]
  \centering
  \caption{Precision \& recall of search results.}  
  \scalebox{1}{
  \begin{tabular}{ |l|cc|cc| } 
    \hline
    & \multicolumn{2}{c|}{\tata} & \multicolumn{2}{c|}{\textit{Base}} \\ \hline
    Local tables & Precision & Recall & Precision & Recall \\
    \hline
    COMPANY  & 0.16 & 0.81   & 0.03 & 1.00\\
    WALMART  & 0.24 & 0.83   & 0.04 & 1.00 \\  
    AMAZON   & 0.19 & 0.82   & 0.07 & 1.00 \\ 
    GAME     & 0.28 & 0.87   & 0.02 & 1.00 \\ 
    MOVIE    & 0.26 & 0.81   & 0.04 & 1.00 \\ 
    CAR      & 0.21 & 0.80   & 0.06 & 1.00\\
    \hline
    \end{tabular}
  }
  \label{tab:effect}
\end{table}
\end{comment}





==> filter.tex <==
\subsection{Task-related table selection}
\label{sec:tab:selection}

\begin{comment}
\begin{table}[t]
  \centering
    \small
  \caption{Example of query text generation patterns}  
  \begin{tabular}{ |l|l|l| } 
    \hline
    Text id & Pattern & Example  \\
    \hline
    Text 1 & Column Names & "Game Name, Year, Genre, Sales"\\
    Text 2 & X + y & "Video game(X) sales(y)"\\
    %Text 3 & X + y + "Prediction"  & "Video game(X) sales(y) Prediction" \\
    \hline
  \end{tabular}
  \label{tab:qtext:generation}
\end{table}

\end{comment}

\begin{comment}
Join row search engine can quickly identify thousands of candidate join rows (tables) from millions of tables in data lakes.
However, it is not a good solution for creating an enriched table by joining all retrieved rows.
Assume that the query table contains 10K rows and for each query row we search the top-10 join rows, thus we will get 100K rows within at least tens of thousands of target tables.
It will be very time-consuming to create a large enriched table with such a large number of candidate tables,
and build the machine learning model.
More seriously, the retrieved target tables also contain many irrelevance tables that
they can join with the query table, but their information cannot contribute to the ML task.
Adding these noise data (columns) will weaken the performance of feature selection algorithms \cite{fs-survey} 
and decreases the accuracy of the ML model.
\end{comment}


There are large numbers of candidate tables after join row search.
It is very time-consuming to create a large enriched table with them.
More seriously, the candidate tables also contain many irrelevance tables that
they can join with the query table, but their information cannot contribute to the ML task.
Adding these noisy data (columns) will weaken the performance of feature selection algorithms \cite{fs-survey} 
and decreases the accuracy of the ML model.
%before joining rows to the query table, 
We propose a further selection to pick up task-related tables.
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/select-crop.pdf}
  \caption{Text-based query and semantic matching.}
  \label{fig:select}
\end{figure}


\begin{comment}
\subsection{Text-based query and semantic matching}
For selecting the tables which are possible to improve the accuracy of the ML task,
we should select the candidate tables which are not only related to the topic of the query table 
but also related to the target variable we want to predict.
For example, there are two target tables, one is about ``video game music", 
and the other one is about ``video game reviews and ratings".
We prefer to select the latter one for predicting the sales of video games 
because the reviews and rating data are correlated to the sales.

Considering the above requirements,
\end{comment}

we formalize this task-related table selection problem as a top-$m$ table retrieve problem with text-based query and semantic matching \cite{ad-hoc-table}. 
The purpose of using a text-based query is to match a related table according to the description of the ML task.
The goal of semantic matching is to go beyond lexical matching by using pre-trained language models to encode both query text and
target text as vectors into a semantic space. 
%Therefore, we transform the top-$m$ table retrieve problem as a top-$m$ vector search problem.

%\subsection{Query text generation}
For a query table,  we allow users to input the description text of their ML task as the query text.
We also propose to generate multiple query texts if the task description text is not available.
The key point is to input the target information (e.g. the "sales" of the video game) into the query text 
so that we can retrieve those tables related to "video game sales" rather than "video game music".
We offer two patterns of query text generation.
Pattern 1 is to use the column names concatenation as query text.
The names of columns contain both the attribute and target information, e.g., "Game Name, Year, Genre, Sales" in the example of video game sales.
Pattern 2 is denoted as X + y, where X is the entity general name of the entity in the table, e.g. "video game",
and y is the target name we want to predict, e.g., "sales".
%Text 3 is more directly that concatenates the term "prediction" after X + y, e.g., "Video game sales prediction",
%for selecting tables that are used in the prediction tasks. In the language model, the synonym of "prediction" will also be considered 
%such as "forecasting", "estimate", and "analysis".

For a target table, we set the attributes $t.title$, $t.context$, and $t.column\_names$ as target texts.
To evaluate the related score of , we take the maximum semantic similarity score between a query text $q_{text}$ 
and all target texts.
Figure \ref{fig:select} gives an image of the semantic matching of the query table with a target table.
There are many ways to aggregate the pairwise scores between encoded vectors, and we take a maximum 
aggregate function in our experiment.
\begin{equation}
    %score(q,t) = max( \sum_{i} score(q_{text}, t_{text[i]}))
    score_{max}(q,t) = max(score(q_{text}, t_{text[i]}))
\end{equation}

\begin{comment}
\begin{equation}
    score_{sum}(q,t) = \sum_{i} score(q_{text}, t_{text[i]})
\end{equation}
\begin{equation}
    score_{min}(q,t) = min(score(q_{text}, t_{text[i]}))
\end{equation}
\end{comment}


We can control the selected table number as $m$ in the top-$m$ table retrieved from the candidate after the join row search.
This helps us to narrow down the number of candidate tables to hundreds of tables and pass them to the next phase of row and column alignment.




==> relatedwork.tex <==
\section{Related work}
%\fixme{re write}
%一般的 related dataset 问题 for different applications but not ML
There are many related works on table retrieval \cite{webtable-ERA-survey, webtables} 
from data lakes and focus on different end tasks such as column and row extension \cite{find-related-table, msj, entitable, concept-expansion}, 
schema matching \cite{table-union-search, table-stitch}, searching joinable tables \cite{josie, pexeso},
table filling \cite{infogather,infogather+}, and knowledge graph building \cite{tablenet, web-table-interpretation}. 
Entity matching \cite{ditto,magellan} is also a similar but different research problem.
It only deals with the case of joining (or matching records from) two given tables; 
it is unknown how to retrieve joinable tables in a data lake, 
and it is prohibitive to try to entity matching every table in the 
data lake with the query table.

For table enrichment for ML, a practical way is to collect and search from the web tables.
We refer the readers to \cite{webtable-ERA-survey} for various methods of table searching and augmentation based on different attributes and end tasks.
There are researches on searching tables with a query keyword \cite{webtables} or a query table.
The InfoGather system \cite{infogather,infogather+} matches tables based on topic-sensitive page rank and semantic graph structure
for table augmentation and column heading discovery.
Tablenet \cite{tablenet} interlinks tables with \textit{equivalent} and \textit{subPartOf} relational types 
for constructing the knowledge graph of tables.
\cite{find-related-table} finds related tables for augmenting the input table with additional rows and columns
based on the aggregated similarity between cell and header values.
The Mannheim Search Join Engine \cite{msj} uses column headings to search candidate tables and rank them by the similarity between cell values.
\cite{josie} searches joinable tables from large-scale tables with the constraint of the exact matching of cell values.
There are also many works on tables' row extension
\cite{entitable,concept-expansion,table-union-search}. 



==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> symbols.tex <==
\begin{table}
  \centering
  %\resizebox{\linewidth}{!}{%
  \begin{tabular}{|l|l|} \hline
    Symbol & Description\\ \hline \hline
    $c$ & collumn\\ \hline
  \end{tabular}
  %}
  \caption{Frequently used notations.} 
  \label{tab:symbols}
\end{table}
